Modulated Neural ODEs

Neural ordinary differential equations (NODEs) have been proven useful for learning non-linear dynamics of arbitrary trajectories. However, current NODE methods capture variations across trajectories only via the initial state value or by auto-regressive encoder updates. In this work, we introduce Modulated Neural ODEs (MoNODEs), a novel framework that sets apart dynamics states from underlying static factors of variation and improves the existing NODE methods. In particular, we introduce $\textit{time-invariant modulator variables}$ that are learned from the data. We incorporate our proposed framework into four existing NODE variants. We test MoNODE on oscillating systems, videos and human walking trajectories, where each trajectory has trajectory-specific modulation. Our framework consistently improves the existing model ability to generalize to new dynamic parameterizations and to perform far-horizon forecasting. In addition, we verify that the proposed modulator variables are informative of the true unknown factors of variation as measured by $R^2$ scores.

==> content/8neurips_reviews.tex <==

\section{General response}
\begin{markdown}
We sincerely appreciate your time and effort in providing valuable feedback. Since our findings and core ideas haven't resonated with you as much as they do with us, we'd like to take this opportunity to first try to better convince you of the overall approach and significance of our work. For specific comments, we have addressed them in the respective "rebuttal" sections.

**Why modulators:** 
Standard NODEs and subsequent works aim to learn a single dynamics function that has a single latent ODE state.  In practice, however, different observations might have different fixed underlying parameterization of the dynamics function or different observed characteristics. Whereas standard methods can only model this variation through a **changing** latent ODE state resulting in a complicated dynamics function that fails to extrapolate (see Fig 2-4, Table 3), Modulated NODEs explicitly accounts for this variation through the time-invariant modulator variables. 

**Benchmarking:** 
We assessed our method on five established NODE benchmarks, enhancing their intricacy by sampling all parameters, incorporating friction, utilizing all digits, adding more walking sequences, and so on. It was striking to observe how easily prior methods, including the state-of-the-art HBNODE, collapsed due to these minor dataset modifications. 
We believe that this highlights a general limitation of earlier methods and affirms the importance of our approach.


**Findings:**
Our method on average improves long-term forecasting test MSE by 55.23\% across all baselines and datasets.  
Moreover, the modulator variables' latent representation offers insights into the true unknown factors of variation: (i) they align closely with the ground truth factors as measured by $R^2$ (Table 3), (ii) they exhibit a similar topology to the observation space (Figure 16, Supp. mat. D). As a consequence, also the latent ODE state is more consistent with the true underlying dynamics: (i) the amplitudes of latent trajectories heavily correlate with the observed sequences (Figures 2-3), (ii) the rotating digit sequences overlap as expected (Fig 4).
In conclusion, our method demonstrably excels at identifying meaningful representations and offers an elegant approach that opens new avenues in dynamic representation learning, given its wide applicability.

**Applicability:**
Our intent was to propose a "simple-yet-effective" solution, enabling easy integration into various NODE models. The empirical results on four NODE variants attest to the immediate advantages our modulator variables offer. We would be pleased if you agree that the simplicity and versatility of our method warrants positive recognition.
\end{markdown}

\section{Reviewer dvMp, rating 4}
\subsection{Weaknesses}
\begin{itemize}
    \item Similar work has been proposed, see https://arxiv.org/abs/2302.13262 
    \item  no clear theoretical guarantees
    \item training difficulties. It would be helpful to see some ablation and show it is easy to train.
\end{itemize}
\subsection{Questions}
\begin{enumerate}
    \item How are the networks trained? There are so many different networks.
    \item Also, how is this method significantly different from existing literature?
\end{enumerate}

\subsection{Response}

\begin{markdown}
Thank you for reviewing our work. Please find below our response to the concerns voiced. 
> How are the networks trained? There are so many different networks. 

We have a simple feedforward architecture,  which we can train easily end-to-end, no more complex than NODE [1] or ODE2VAE [2]. Specifically, MoNODE optimizes ELBO like NODE, that is the optimization of the additional modulator encoder networks is implicit, with no extra loss terms:
\end{markdown}
\begin{align}
    \log p(X) & \geq \textup{ELBO} = \sum_n \mathbb{E}_{q_{\boldsymbol{\nu}}} \left[  \log p\big(\mathbf{x}_{1:T}^{n} \mid \mathbf{z}_1^{n} \big)  \right] - \textup{KL}\left[ q_{\boldsymbol{\nu}}(\mathbf{z}_1^{n}\mid\mathbf{x}^n_{1:T_z}) \| p(\mathbf{z}_1) \right].
\end{align}
We would like to clarify that there are only 3 networks in the proposed method: two of which are the standard building blocks of a VAE (encoding, decoding network) as in [1] and the third, our addition, the modulator prediction network. We explicitly name the networks to clarify the intuition, following the narrative style of ODE2VAE [2].

[1] Chen, R. T., Rubanova, Y., Bettencourt, J., \& Duvenaud, D. K. (2018). Neural ordinary differential equations. Advances in neural information processing systems, 31.

[2] Yildiz, C., Heinonen, M., \& Lahdesmaki, H. (2019). ODE2VAE: Deep generative second order ODEs with Bayesian neural networks. Advances in Neural Information Processing Systems, 32.

\begin{markdown}
 > It would be helpful to see some ablation and show it is easy to train.

The proposed model is very easy to train, and not sensitive to hyperparameters. Our model performs consistently well under different hyperparameterization:

(i) the solver used (Table 9., Supp. mat. D); 

(ii) the number of input frames $T_z$ used (Table 10., Supp. mat. D); 

(iii) the latent dimensionality of the latent ode state $q_z$ and modulator variable $q_s$ (Table 11., Supp. mat. D). 

In addition, to showcase that our proposed framework is easy to train we have plotted the validation MSE versus wall clock time during training for sinusoidal data, please see Figure 1 (additional PDF, global response). As it as apparent from the figure, our framework is easier to train than all baseline methods. We realize that these ablations were not easily accessible, so we will move a highlight of them to the main paper.

\end{markdown}

\begin{markdown}
> no clear theoretical guarantees

Similarly to earlier works in this area of research like ODE2VAE [2], LatSegODE [3] and Neural Event ODE [4], we introduce an additional structure on top of the flexible neural ODE model class without a theoretical investigation. Nonetheless, we show empirically that in practice our framework brings a significant accuracy improvement with an average of 55.25\% across all experiments, and a high of 88.38\% improvement on PP dataset. We leave a theoretical study as a fantastic next step for future work, to explore the limits of our ideas, especially with respect to the complexity of the static signal.

[3] Shi, R., & Morris, Q. (2021, July). Segmenting hybrid trajectories using latent odes. In International Conference on Machine Learning (pp. 9569-9579). PMLR.

[4] Chen, R. T., Amos, B., & Nickel, M. (2020). Learning neural event functions for ordinary differential equations. arXiv preprint arXiv:2011.03902.

\end{markdown}

% our design is driven by intuition. Specifically, separating the static from the dynamic signal, then modelling dynamics based on the dynamic signal only.
% The hope with our intuition was that the static-dynamic separation will allow for better temporal modelling and all benefits thereafter (better temporal extrapolation, generalization), as the correlations will span a significantly smaller subspace (rotations are a 1-parameter group, even if they happen in thousand-dimensional inputs), as also corroborated in practice.
% A theoretical study is a fantastic next step that we leave for future work, to explore the limits of the intuition, especially with respect to the complexity of the static signal.


\begin{markdown}
> Also, how is this method significantly different from existing literature?

We compare with a great array of state-of-the-art methods, a visual summary is in Table 1 in the main paper. Our method is significantly different from the existing methods as 

(i) we introduce modulator variables that allow the model to preserve core dynamics while being adaptive to modulating factors. This, in turn, allows us to model underlying factors of variation that are fixed in time.

(ii) our framework addresses a common limitation of existing NODE type models: poor long-term forecasting performance; 

(iii) our modulator variables are informative of the true unknown factors of variation as measured by $R^2$ scores; 

(iv) it is a *general* framework that can be combined with a large variety of existing NODE type models, bringing on average across all experiments 55.25\% accuracy improvements.

> similar work has been proposed, see https://arxiv.org/abs/2302.13262

We do appreciate your knowledge of the related work, even of its newest additions. As you might have noticed, this arxiv submission is very related to ours and we are very aware of it. On the other hand, the paper isn't published yet, and we have very good reasons not to cite it.

\end{markdown}

% We are the first to introduce the novel concept of modulator variables for Neural ODE models.

% On top of this, we enforce that these parameters are time-invariant.
% As such, improving generalization and forecasting as shown experimentally for many dynamical systems. 



\section{Reviewer 8J7y, rating 5}
\subsection{Weaknesses}
\begin{itemize}
    \item They experimented by dividing 5.1 dynamics modulator variable and 5.2 static modulator variable data to evaluate their modulators, but they could not show whether each modulator actually played its role.
\end{itemize}
\subsection{Questions}
\begin{enumerate}
    \item Was the dynamics modulator also applied to static variables in these experiments? If the dynamics modulator was used even in the static variable experiment, you should remove the dynamics modulator. If you did not use dynamics modulator in static variable experiment, you should experiment using dynamics modulator. In other words, through these experiments, it is necessary to check whether each modulator is playing a role.
\end{enumerate}
\subsection{Response}
\begin{markdown}
Thank you for the review, please find below our response to the concerns voiced.
> Was the dynamics modulator also applied to static variables in these experiments? If the dynamics modulator was used even in the static variable experiment, you should remove the dynamics modulator. If you did not use dynamics modulator in static variable experiment, you should experiment using dynamics modulator. In other words, through these experiments, it is necessary to check whether each modulator is playing a role.

To confirm the role of each modulator variable we have performed 2 additional ablations with the MoNODE framework on: (a) Sinusoidal data with static modulator instead of dynamics; and (b) rot. MNIST with dynamics modulator instead of static.  We report the test MSE across 3 different initialization runs with standard deviation. For Sinusoidal data for MoNODE + static mod. the test MSE performance drops to 2.68 (0.38) from MoNODE + dyn. mod. 0.29 (0.11). For Rot. MNIST MoNODE + dyn. mod. the performance drops to 0.096 (0.008) from MoNODE + static mod. 0.030 (0.001). In addition, we examined the latent embeddings of the dynamics modulator for Rot. MNIST. Where previously for the content modulator we observed clusters corresponding to a digit's class (Fig. 16, Supp. mat. D), for dynamics modulator such a topology in the latent space is not present, see Fig. 2 (additional PDF, general response). In all, the results confirm that the modulator variables are correlated with the true underlying factors of variation as indicated by the obtained $R^2$ scores (Table 3., main paper) and latent embedding plots (Fig. 16, Supp. mat. D), and, as such, play their corresponding roles.  
\end{markdown}


% To demonstrate the benefits of our modulated framework, we design synthetic experiments where we can control the true underlying static and dynamic variables. We further assume to know whether the dataset of our interest is modulated by static or dynamic variables. We believe it is viable to have such minimal prior knowledge about an observed system (e.g., "extinction rates in prey-predator populations could differ across observed populations" or "different people would have different walking styles"). In turn, such prior knowledge lets us include the corresponding network in our framework, meaning that we never apply dynamics modulators to infer static modulator variables.

% The proposed framework came about from a practical observation that in many instances (i) the underlying dynamics function is the same, only the parameters vary (dynamics modulators), and (ii) the physical representation of the object is also left unchanged (static modulators). Therefore, we introduced the modulator framework as a practical approach to account for these factors. To confirm our intuition that the proposed method brings performance improvements we design synthetic experiments where we can control what are the true underlying static and dynamic variables. In the case for section 5.1 the underlying data is low-dimensional, the actual coordinates of the data points, therefore, there is no need for a static modulator variable as there are no physical characteristics of the object itself (color, shape, etc.). Likewise, for section 5.2, the underlying dynamics are fixed, therefore there is no need for a dynamics modulator variable (parameters of a differential equation) as the function is left unchanged. Consequently, in each of these section we only use either the dynamics modulator (section 5.1) or static modulator (section 5.2). 


% We measure in fact the contribution of the static and dynamic variables, in isolation and jointly, in Tables XX, XX, XX.
% Key results:
% 1.
% 2.
% 3.

% All experiments demonstrate that including correct inductive bias (i.e., dynamics modulator variable if the dynamics function is controlled, or static modulator variable if observation mappings are sequence-specific) significantly improves model performance.

% To further nail the conclusion and ground it to real settings, we experiment with the real-world Mocap with human-skeletons walking.
% By human anatomy, physical characteristics like leg length, shoulder width, etc, directly impact the dynamics of walking.
% Interestingly, traditional modeling with a single latent space (NODE, ...) has considerably worse than MSE which models the same signal but separated into a temporal and a static component (table XX).
% Obviously, using only the dynamic or only the static in an ablation (table XX), is not failing but also not as accurate.


% We further evaluate the added benefit of each modulator variable in section 5.3 by a Mocap experiment. This is a real world dataset, where by intuition both variables should play a role. The length of a person's legs should affect walking speed (dynamics modulator), however, shoulder width, etc. should affect the reconstruction quality (static modulator). To investigate the benefit of each modulator we perform an ablation where we evaluate the test MSE performance when only one of the modulator variables is present versus both. As reported in table 12 in supplementary material D, Additional results, having both variables brings the best performance as indicated by the lowest test MSE. The choice of which is modulator variable to include could be seen as an inductive bias that comes as expert knowledge of the observed data at hand. 

% > they could not show whether each modulator actually played its role.

% For dynamics modulators: we evaluate whether the learned dynamics modulator 'played its role' by computing how much information the latent representations carry about the true parameters. As described in Schott et al. 2021 we compute $R^2$ scores by performing regression from latent variables to the true parameters. The regression input for MoNODE are the inferred dynamics modulators, while for NODE it is the latent trajectories. For all experiments in section 5.1, sinusoidal, predator-prey and bouncing ball with friction, our proposed framework obtains significantly high $R^2$ scores, implying that the learned dynamics modulators are informative about the underlying parameters of the system. We remind that in the same vein as NODEs, our latent model does not allow for interpreting individual parameters.

% For static modulators: we evaluate the static modulator embedding space and the state trajectories for the rotating MNIST experiment. We first observe that the learned dynamics lead to cyclic trajectories, matching the pattern in the high-dim observed sequences. Further, in figure 16., supplementary material D, we see that, even though we have not explicitly enforced any topology in the latent vector space, we can observe clustering of the data points corresponding to a given digit style (0 versus 1 for example). This qualitative observation indicates that the static modulator has captured information of the underlying characteristic of the observations. Albeit, the separation of the clusters is not perfect, the explanation of this is two-fold: visually examining the data points it can be seen that some digits from different classes look very similar due to the handwriting, and we have not enforced in the latent space that each digit class should be embedded as far as possible from each other, hence the observed overlap is reasonable. 



\section{Reviewer VxYT, rating 5}
\subsection{Weaknesses}
\begin{itemize}
    \item As the output of the static modulator and the dynamics modulator is used by concatenation, I would like to see the experimental results without the static modulator or the dynamics modulator to determine if they are both essential.
    \item I would like the authors to add the inference time cost comparison with and without those modulators.
\end{itemize}
\subsection{Response}
\begin{markdown}
Thank you for reviewing our work, please find below the response to the concerns voiced. 

> As the output of the static modulator and the dynamics modulator is used by concatenation ...

We never concatenate static and dynamic modulators. They are additional inputs to the decoder and differential function, respectively. We do concatenate the dynamic state $z$ and each modulator variable separately.

> ... I would like to see the experimental results without the static modulator or the dynamics modulator to determine if they are both essential.

We do not always use both modulator variables, but rather the one(s) that match the problem: 

(i) for low-dimensional problems with changing dynamic's parametarization we use **only** dynamics modulator (Section 5.1)

(ii) for high-dimensional problems with changing object features, but fixed dynamics, we use **only** static modulator (Section 5.2) 

(iii) for problems that have both, changing dynamic's parametrization and changing object features, we use **both** modulator variables (Section 5.3)

That said, we investigated the utility of using both modulator variables versus only one for Mocap (Section 5.3). Using both modulator variables resulted in the lowest test MSE as compared to using only one, either static or dynamics modulator, as reported in Table 12 (Supplementary material D, Section 'Additional results'). This performance gap can be attributed to the data, which contains both static (length of limbs) and dynamics (length of legs) modulating signals, therefore, both variables are needed for optimal performance. 

If for problems (i) and (ii) the corresponding modulator is switched to the opposite ((i) Sinusoidal data with static modulator instead of dynamics; and (ii) rot. MNIST with dynamics modulator instead of static) we see a drop in performance with respect to test MSE. Specifically, for Sinusoidal data for MoNODE + static mod. the performance drops to 2.68 (0.38) from MoNODE + dyn. mod. 0.29 (0.11). For Rot. MNIST MoNODE + dyn. mod. the performance drops to 0.096 (0.008) from MoNODE + static mod. 0.030 (0.001). In all, this confirms that the modulator variable selection is essential, depends on the problem at hand and our framework can accommodate multitude of problem set-ups. 
\end{markdown}

% To answer this we focus on our synthetic experiments, where we control the data ((e.g., fix extinction rates in prey-predator populations across runs), and importantly, we can define if the dataset is modulated by static and/or dynamic modulators. Therefore, we include the modulator variable(s) matching the problem (as described in great detail in sections 5.1 and 5.2).

% Beyond the synthetic experiments, in the real-world MOCAP dataset both static and dynamic signals are present and we cannot ablate on them explicitly.
% That said, we investigate the utility of using both modulator variables versus only one for Mocap also.
% % We expect intuitively that although both variables are beneficial, perhaps using only one is sufficient.
% Using both modulator variables instead of just one is beneficial as indicated by the lowest test MSE (table 12, supplementary material D, section 'Additional results').
% This is expected, since in the real-world Mocap both static and dynamic signals are within the data and omitting one of them deprives the model of important information.

% We only do such a comparison for mocap dataset as the other datasets by design only have one underlying factor of variation, either the dynamics parameters (section 5.1) or the object characteristics (section 5.2). As such, deciding whether to include both or one modulator variable is a design choice based on the underlying data at hand.  

\begin{markdown}
    
> I would like the authors to add the inference time cost comparison with and without those modulators.

We compute the inference time cost for the Sinusoidal data experiment, where the test data consists of 50 trajectories of length 150. We record the time it takes NODE and MoNODE to predict future states while conditioned on the initial 10 time points. We perform the evaluation 10 times and report the mean (in seconds) and std. The inference time cost for NODE is 0.312 (0.050), while for MoNODE is 0.291 (0.040). We are faster because the number of parameters for MoNODE is lower than for NODE, 24598 versus 24666, respectively. As such, we would like to highlight that the inference time costs of our framework is on par with the base models where the exact time is dependent on the total number of parameters, which is comparable between all base and Mo*NODE models (Table 7., Supp. mat. C). We will add these results to the final version. 
    
\end{markdown}

\section{Reviewer m2DA, rating 6}
\subsection{Questions}
\begin{enumerate}
    \item Is there a way the modulations spaces could be used for interpolation between different systems?
    \item Could this work be extended to process PDE equations?
\end{enumerate}
\subsection{Response}
\begin{markdown}
Thank you for the review, please find below our response for the questions voiced.

> Is there a way the modulations spaces could be used for interpolation between different systems?

Thank you for the interesting question. It touches upon a possible Bayesian extension of the presented work. In particular, in the current set-up the modulator variables are point estimates, however, this could be adjusted to learning possibly multi-modal modulator variable distributions. Ideally, each mode of the inferred posterior could correspond to a particular system (e.g., a handful of particles with no/weak/strong interactions). That being said, the completely black-box nature of our framework could make it difficult to interpret/identify modulators and therefore the systems.

> Could this work be extended to process PDE equations?

Based on the recent work on neural PDEs [1], it is possible to parameterize the systems of ODEs resulting from spatial discretization of a PDE in the same way as our framework. An interesting research question would be, for instance, learning modulators as a function of spatial coordinates. 

[1] Learning Space-Time Continuous Neural PDEs from
Partially Observed States. Iakovlev, Heinonen, Lähdesmäki, 2023.

\end{markdown}
% However, we must admit that PDEs are out of our expertise; hence, we are unable to answer this question in full confidence.

\section{Reviewer Y7gY, rating 4}
\subsection{Weaknesses}
\begin{itemize}
    \item Experimental examples are not convincing enough.
    \item It is not clear whether the slight improvement in performance is due to the additional number of parameters.
    \item paper does not directly provide a visual presentation or intuitive explanation of the static and dynamics modulator variables extracted by the modulator prediction networks.
\end{itemize}
\subsection{Questions}
\begin{enumerate}
    \item  When comparing with NODE, could you provide a comparison of the number of parameters and set up a more reasonable experiment to prove that the performance improvement is not caused by the increase in the number of parameters?
    \item Whether the MoNODE framework can outperform the conventional NODE on the task of learning more complex dynamical systems, such as trajectories generated by a family of chaotic systems controlled by different parameters?
    \item For the CMU Mocap datasets, due to the addition of the modulator variables, the MoNODE is supposed to significantly improve the performance of NODE in the Mocap-Shift task, but in fact, the improvement effect is not obvious, which is far less than that of Mocap. Can you further explain this phenomenon?
    \item Could you directly provide some visual description and intuitive interpretation of the modulator variables extracted by the modulator prediction networks?
\end{enumerate}

\subsection{Response}
\begin{markdown}
Thank you for the detailed review. Please find below our response to the concerns voiced. 

> Experimental examples are not convincing enough.

We are slightly surprised and sorry to hear that our findings fail to convince the reviewer. We exhaustively test our ideas on four NODE variants (standard, SONODE, HBNODE, LSONODE) on five datasets that were all previously used to evaluate similar approaches. Our Mo*NODE framework improved by 88.38\% test MSE for PP experiment and on average by 55.25\% across all experiments, as reported in Table 2. and Table 4. That being said, we would be happy to know what other experiments would help us convince the reviewer.

> When comparing with NODE, could you provide a comparison of the number of parameters and set up a more reasonable experiment to prove that the performance improvement is not caused by the increase in the number of parameters?

Thank you for voicing this concern, as indeed one candidate explanation for the observed performance improvement could be increased parameter count. To account for this fact we approximately match the number of parameters in the base network and the Modulated counterpart. For a complete overview of the number of parameters of each model for each experiment please see Table 7 in the supplementary material, Section C, Architecture and Hyperparameter Details. In particular, for sin, PP, and BB, NODE model actually has a higher parameter count than its MoNODE counterpart (We also control overfitting by choosing the best model via cross-validation). Furthermore, to also account for the fact that the performance boost is not caused just by a larger latent dimensionality, we match the latent dimensionality between the base model and the modulated counterpart. As such, we are confident to say that the observed performance boost is not caused simply by an increase in number of parameters, but rather by the framework itself. 

> Whether the MoNODE framework can outperform the conventional NODE on the task of learning more complex dynamical systems, such as trajectories generated by a family of chaotic systems controlled by different parameters?

We perform an additional ablation on a Lorenz Attractor dataset, with varying parameters as suggested. MoNODE outperforms NODE on both short- and long-horizon forecasting. Specifically, the test MSEs for NODE and MONODE are 36.19 vs 33.90 for short term and 61.28 vs 46.56 for long term. We would like to remind that NODEs are known to suffer from solver stability issues on chaotic systems [1].

[1] Experimental study of Neural ODE training with adaptive solver for dynamical systems modeling

% We perform an additional ablation on a Lorenz Attractor dataset, where the parameters $\rho$, $\sigma$, $\beta$ are sampled from the corresponding Normal distributios: $\rho \sim N (29.0, 0.8)$, $\sigma \sim N(10.0, 0.8)$, and $\beta \sim N(2.67, 0.8)$. The initial condition is fixed at $x,y,z=(1.0,1.0,1.0)$. We generate $N_train = 2000$ of length $T_train=T_valid=1000$, $N_valid=N_test=200$ and $T_test=3000$. The number of parameters for NODE is 31378, while for MoNODE 29354. MoNODE outperforms NODE on both short- and long-horizon forecasting (T=1000 and T=3000). Specifically, the test MSE for T=1000 for NODE is 36.19 (5.94) while for MoNODE 33.90 (4.93) and for T=3000 for NODE 61.28 (4.47) and for MoNODE 46.56 (6.91). 

> For the CMU Mocap datasets, due to the addition of the modulator variables, the MoNODE is supposed to significantly improve the performance of NODE in the Mocap-Shift task, but in fact, the improvement effect is not obvious, which is far less than that of Mocap. Can you further explain this phenomenon?

% We were also surprised by this outcome and attributed it to our data splitting.

This outcome can be attributed to the chosen data splitting. In particular, we choose to leave a particular subject out for testing since the other subjects had either too many or too few sequences (notice that leaving out a subject with too many/few sequences would lead to a huge decrease in the training data size or biased testing). Thanks for raising your concern, we will include a detailed explanation for this situation in our paper.

> Could you directly provide some visual description and intuitive interpretation of the modulator variables extracted by the modulator prediction networks?

Dynamics modulators: intuitively they capture information about the true underlying differential equation parameters (experiments sin, PP, BB) or in the case when the dynamic's function in closed form is unknown (Mocap), then the parameters that affect this unknown function (length of legs). 

To confirm that this intuitive explanation indeed holds, we computed the $R^2$ scores by performing regression from latent variables to the true parameters, as described in Schott et al. 2021. The regression input for MoNODE are the dynamics modulators, while for NODE it is the latent trajectories. For all experiments in Section 5.1, sinusoidal, predator-prey and bouncing ball with friction, our proposed framework obtains a higher $R^2$ score (a score of 1 corresponds to perfect regression) implying that the learned dynamics modulators have captured information of the underlying parameters of the system.

Static modulators: intuitively they capture static characteristic features of the data, in the case when the data is image sequences, for example. In this case, the static modulator would capture the color, shape and other static features of the moving object.

To assess whether this assumption is true we evaluate the learned vector space of the static modulator for the rotating MNIST experiment. In particular, in Figure 16., Supplementary material D, Additional results, we see that, even though we have not explicitly enforced any topology in the latent vector space, we can observe a clustering of the data points corresponding to a given digit style (0 versus 1 for example). This qualitative observation indicates that the static modulator has captured information of the underlying characteristic of the observations. Albeit the separation of the clusters is not perfect, the explanation of this is two-fold: visually examining the data points it can be seen that some digits from different classes look very similar due to the handwriting, and we have not enforced in the latent space that each digit class should be embedded as far as possible from each other, hence the observed overlap is reasonable. 

We will provide a sufficient visual description in the final version of the paper.
\end{markdown}

% Initially we were also surprised by this outcome, however, examining it more closely this is rather a bug of NODE than MoNODE. Specifically, we can see that for MoNODE the performance for both Mocap and Mocap-Shift is largely unchanged, while for NODE we seem to observe a performance boost for Mocap-shift. For us this suggest that the individual left out as the test case for Mocap-shift might be highly representative of the dataset itself, thus, explaining NODE improved performance, while for MoNODE the performance on a completely unseen individual is on par when samples from all are observed. Meaning that our framework is more robust to generalizing to unseen parameterisations as confirmed by the lower test MSEs in all experiments. 


\section{Reviewer Znd9, rating 4}
\subsection{Weaknesses}
\begin{itemize}
    \item it is not entirely clear whether the proposed model can effectively capture the time-invariant aspects of observations over an arbitrary time span.
    \item similarly, the proposed model requires the observation of length $T_e$ to predict the time-invariant modulating variables. Therefore, it is not greatly applicable for the case when $T_z < T_e$ .
    \item The paper lacks a comparison with a relevant previous work [1], which factorizes the latent space into content and motion variables and models the dynamics using the (Hamiltonian) latent NODE. ([1] Khan, A., \& Storkey, A. J. Hamiltonian latent operators for content and motion disentanglement in image sequences. NeurIPS 2022.)
\end{itemize}
\subsection{Questions}
\begin{enumerate}
    \item I think it would be great to experimentally demonstrate that a trained modulating prediction network indeed guarantees time-invariance in the long-term time horizon. For example, it would be helpful to plot a graph to visualize the change in or over time (ideally to be a constant line). 
    
    \item Is the performance of the trained MoNODE still good when $T_z = T_e << T_train$ It seems that an ablation study is needed to check this.

    \item  I am curious whether MoNODE would be applicable to chaotic dynamics. For instance, one could consider the parameters of the Lorenz system as dynamic modulating variables. Can MoNODE effectively learn and infer them?

    \item Max pooling [2] is commonly used as the pooling function for invariant mappings (e.g., for the static modulator case). Is there a specific reason for using averaging? It would be nice if the authors could conduct a comparison between max and average pooling invariant maps.
\end{enumerate}

\subsection{Response}
\begin{markdown}
Thank you for the detailed review, please find below our response to the concerns voiced. 
> I think it would be great to experimentally demonstrate that a trained modulating prediction network indeed guarantees time-invariance in the long-term time horizon. For example, it would be helpful to plot a graph to visualize the change in or over time (ideally to be a constant line). 

We would like to clarify that the modulator prediction network does not guarantee time-invariance with respect to the predicted dynamic state $z$, but rather the modulator variables $d$ and $s$. Our proposed framework accumulates prediction error as commonly known with auto-regressive frameworks, yet minor compared to the existing base models (NODE, SONODE, HBNODE, LSONODE) as shown in Figures 2-3 and Figures 10-15 (Supp. mat. D) and indicated by the accuracy improvement with respect to test MSE: Sin by 84.47 \%, PP by 88.38 \%, BB by 20.12 \%, Rot.MNIST by 23\%, and MOCAP by 20.08\%.

> Is the performance of the trained MoNODE still good when $T_z = T_e << T_train$ It seems that an ablation study is needed to check this.

In general, the choice of $T_e$ (number of timepoints used for learning modulator variables) is independent of $T_train$ (total training sequence length) but rather depends on the underlying dynamical system's properties. Specifically, a subsequence of length $T_e$ has to have sufficient information of the change in dynamics to correctly estimate the system parameters. Hence, if the underlying dynamics are changing very slowly, a higher number of timepoints (larger $T_e$) are needed to estimate the underlying parameters.
Secondly, the performance of MoNODE is good when $T_z = T_e$. As reported in Table 7 (Supp. mat., C) for most datasets these two parameters are matched and additional ablations are reported in Table 10 (Supp. mat. D). 
Lastly, we have paid detailed attention to match $T_z$ of NODE with $T_e$ of Mo-*NODE to make sure that the performance boost is not simply caused by a longer input sequence. 

\end{markdown}

% We always choose $T_e < T_train$. The performance of MoNODE is good when $T_z = T_e$. For most datasets these two parameters are matched for Mo-*NODE models as reported in Table 7 (we also performed additional ablations on different parameters $T_z$, $T_e$ as reported in Table 10.

\begin{markdown}
> similarly, the proposed model requires the observation of length $T_e$ to predict the time-invariant modulating variables. Therefore, it is not greatly applicable for the case when $T_z < T_e$.

Our framework is applicable to settings when $T_z < T_e$. Please see Table 10. (Supp. mat. D), where our framework outperforms base models also when $T_z < T_e$. 

\end{markdown}
% That said, of course they may exist corner settings and datasets where indeed this is not the case, as with most methods and their hyperparameters.
% We also agree with the reviewer that, as with any other hyperparameter, $T_e$ could potentially prevent us from successfully learning time-invariant variables. Yet, the same limitation applies to all other NODE methods: in the presence of sequence-specific factors of variations (such as the frequency of an observed oscillating sequence), standard methods such as NODE must incorporate information about the underlying factor in their dynamic states $z_t$ as they do not include additional modulating variables. Since the dynamics states are extracted from the first $T_z$ time points, $T_z$ should be sufficiently high for these methods as $T_e$ for our method.

\begin{markdown}
> I am curious whether MoNODE would be applicable to chaotic dynamics. For instance, one could consider the parameters of the Lorenz system as dynamic modulating variables. Can MoNODE effectively learn and infer them?

We perform an additional ablation on a Lorenz Attractor dataset, with varying parameters as suggested. MoNODE outperforms NODE on both short- and long-horizon forecasting. Specifically, the test MSEs for NODE and MONODE are 36.19 vs 33.90 for short term and 61.28 vs 46.56 for long term. We would like to remind that NODEs are known to suffer from solver stability issues on chaotic systems [1].

[1] Experimental study of Neural ODE training with adaptive solver for dynamical systems modeling


> Max pooling [2] is commonly used as the pooling function for invariant mappings (e.g., for the static modulator case). Is there a specific reason for using averaging? It would be nice if the authors could conduct a comparison between max and average pooling invariant maps.

We performed an additional ablation with Max pooling [2] operator instead of averaging for the static modulator on the rotating MNIST experiment and for the dynamics modulator on the sinusoidal data experiment. We report the obtained test MSE across 3 runs with different initialization seeds and corresponding standard deviation. For MoNODE + max pooling on rotating MNIST we obtain test MSE of 0.035 (0.004), which is  better than the baseline model NODE 0.039 (0.003) but is worse than MoNODE + averaging 0.030 (0.001). For MoNODE + max pooling on sinusoidal data we obtain test MSE of 0.28 (0.03), which is on par with MoNODE + averaging 0.29 (0.11) and better than the base model 1.84 (0.70). We chose the averaging operator in our work as modulator variables should capture features that remain constant in time, however, other functions are also a viable option, for example, one could also consider summation [3].

[3] Franceschi, J. Y., Delasalles, E., Chen, M., Lamprier, S., & Gallinari, P. (2020, November). Stochastic latent residual video prediction. In International Conference on Machine Learning (pp. 3233-3246). PMLR.

>  The paper lacks a comparison with a relevant previous work [1], which factorizes the latent space into content and motion variables and models the dynamics using the (Hamiltonian) latent NODE. ([1] Khan, A., \& Storkey, A. J. Hamiltonian latent operators for content and motion disentanglement in image sequences. NeurIPS 2022.)

The code base for [1] unfortunately is incomplete. However, in Section 3.5 of [1] they also perform an experiment on Rotating MNIST (single digit), where ODE2VAE outperforms their method. In our work, we also compare our framework to the non-Bayesian version of ODE2VAE under the name of LSONODE (Section 5.1). Therefore, we perform an additional ablation of ODE2VAE performance on our implementation of Rotating MNIST experiment (all digits) with MoODE2VAE. We report the mean across 3 runs with std. The test MSE for ODE2VAE is 0.068 (0.002), while MoODE2VAE obtains 0.035 (0.002) outperforming ODE2VAE by a large margin. As such, we are confident to say that our method improves the current state-of-the-art and we will contact authors of [1] to include a complete comparison in the camera ready version. 


\end{markdown}






==> content/8reviews.tex <==

Papers positioning: introduce framework of invariance. Focus on ODEs (odes and random odes).

Run experiment with fewer hidden units. (goal: match NODE to INODE size) 

\section{Concerns by AC}
\begin{enumerate}
    \item The experimental section is weak for an empirical paper, since the evaluation of interesting real-world problems is missing. Reviewer aHNa points out that a comparison to more recent Neural ODE models is missing. (In my experience, a standard Neural ODE (using RK4) should perform better on both the sinusoidal and Lotka-Volterra dataset, but research code to reproduce and/or verify the experimental results is missing.) 

    \textbf{Planned Action:}
    \begin{enumerate}
        \item Experiments: Showcase ideas applicability to different NODE type models. 
        
        \begin{itemize}
            \item Works with first order ODEs Latent NODE (Chen 2018)
            \item works with second order ODEs SONODE (2021)
            \item \textit{SDEs?}
            \item \textit{GP-ODEs?}
            \item \textit{works with Random ODEs (Cagatay), latent NODE + extra factors}
        \end{itemize} 
        How to depict: table model vs model + our method.
  %GP-ODEs?.  Aka first showcase that Latent NODE, SONODE, etc fail. 
        \item Text: Mention in text that the focus is on Latent NODE models, where we confirm the results by Rubanova, that the model fails on long term forecasting. And showcase the improvements (a). 
        \item Experiments: clear ablations. Model + euler, rk4, dopri5 etc. 
        \item Text: Paragraph in related work highlighting how our method compares to the existing NODE papers (HBNODE, AGNODE, CNODE, etc)
        \item Text: Paragraph highlighting that our method can be added to existing NODE models with benefits
        \item Experiments: real-life application? (some real life data, maybe from SONODE already used), MOCAP data? (high-dim, hence, why needed latent modelling) (Physionet from Latent NODE?) need to think more on this
        \begin{itemize}
            \item MoCap: multiple sequences, a content variable for person (Cagatay tested with INODE), task: forecasting motion (comparison with NODE vs INODE)
            \item test on a new subject (person) (within distribution) 
            \item content variable 
        \end{itemize}
    \end{enumerate}
    Feedback: 
    \begin{itemize}
        \item re-explain why we don't use certain models in the experiments section.
        \item 
    \end{itemize}
    
    
    \item A table in the main text would help to better contextualize the performance difference between the models. It is not always clear whether INODE or SINODE performs better by just inspecting at the Figures.

    \textbf{Planned Action:}
    \begin{enumerate}
        \item Text: Create a table with comparison (see point a above)
        \item Experiments: Perhaps drop SINODE if no benefit seen
    \end{enumerate}

    
    \item It is difficult to follow the conducted ablation study. An extended ablation study and a better discussion would help to better disentangle the effects of the different proposed innovations.

    \textbf{Planned Action:}
    \begin{itemize}
        \item Experiments: Plot running error overtime (see SONODE for comparsion)
        \item Experiments: Ablations with different numerical solvers (point 1.(b))
    \end{itemize}

    
    \item Reviewer r94C points out that the clarity of the writing needs to be improved in order to better understand the mechanics of the proposed models. Also, the discussion of the contributions is fuzzy, and can be improved.

    \textbf{Planned Action:}
    \begin{enumerate}
        \item Text: Change the variables names section 3
        \item Text: Improve the discussion
    \end{enumerate}
    
    \item In the abstract you claim that your approach enables robust Neural ODE models, but it remains open what is meant by robustness. The term robustness is used in different contexts in this paper. Empirically you show that the model is insensitive with respect to the tuning parameter, but this does not imply that a model is robust. Then you state that the model is somewhat robust to the latent dimensionality, but it is not exactly clear what this means.

    \textbf{Planned Action:}
    \begin{enumerate}
        \item Text: Clarify that our model is focused on long term prediction (which is what we refer to as robustness) \textit{Clarification: generalize across different time series (make link to meta learning, different tasks)}
        Check if other papers generalize to unknown parameter settings. 

        None of the previous works, have investigated model robustness to different parameterization of the differential equation. For example, for sinusoidal data in \citet{rubanova2019latent} the amplitude is fixed for all sequences. In \cite{norcliffe2020second}, a second order NODE (SONODE) model, the robustness is tested with respect to different noise settings for sinusoidal data, however, all trajectories have the exact same parameters of the differential equation. 
        
        
        In \cite{xia2021heavy}, Heavy-Ball NODE, the model performs only one-step ahead prediction, meaning that ground truth data is necessary for every time point, therefore, the model is not applicable for extrapolation. 
        
        In our work we show that the existing methods fail 

        Even though CDE, ANODE (both do classification)
        
        \item \textit{Experiments: out of distribution parameters (decide later on depending on time) }
        \item Experiments: again, perhaps drop the sinode if we have no improvement
    \end{enumerate}
    
\end{enumerate}

